An Efficient Implementation of Riemannian Manifold Hamiltonian Monte Carlo for Gaussian Process Models

This technical report presents pseudo-code for a Riemannian manifold Hamiltonian Monte Carlo (RMHMC) method to efficiently simulate samples from $N$-dimensional posterior distributions $p(x|y)$, where $x \in R^N$ is drawn from a Gaussian Process (GP) prior, and observations $y_n$ are independent given $x_n$. Sufficient technical and algorithmic details are provided for the implementation of RMHMC for distributions arising from GP priors.

==> gpc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Gaussian Process Classification}\label{sec:gpc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As a first evaluation of ARM,
we consider a Gaussian Process (GP) classification model (GPC).
A GP specifies a prior distribution on functions $x : \bxi \to \mathbb{R}$, so that its values $x_n = x(\bxi_n)$ are correlated through a prior covariance matrix $\K$ that depends on the inputs $\bxi_n$.
%
In a GPC model an observed class label $y_n \in \{ -1, +1 \}$ depends on $x_n$
through a likelihood $p(y_n | x_n) = \Phi(y_n x_n)$,
the probit link function being $\Phi(x) = \int \Theta(z) \Ncal(z ; x, 1) \, \drm z$.
The step function $\Theta(z)$ is one if its argument is nonnegative, and zero otherwise.
%
Using the step function, the joint model is $p(\x, \z, \y) = \prod_n \Theta(y_n z_n) \, \Ncal(z_n ; x_n, 1) \cdot \Ncal(\x ; \0, \K)$, and we are interested in the marginal likelihood $Z = p(\y)$
as a function of $\K$.
Two representations of $Z$ arise from either integrating out $\z$ to give
%
\begin{align} 
p(\x | \y) & = \textstyle{ \frac{1}{p(\y)} \exp ( -\frac{1}{2} \x^T \K^{-1} \x } \nonumber \\
& \qquad\qquad\qquad \textstyle { + \sum_{n=1}^{N} \log \Phi(y_n x_n) + c_1 ) } \label{eq:gpc-x}
\end{align}
%%
with
$c_1 = \frac{N}{2} \log 2 \pi - \frac{1}{2} \log |\K|$,
or integrating out $\x$ to yield
\begin{align} 
p(\z | \y) & = \textstyle{ \frac{1}{Z} \exp ( -\frac{1}{2} \z^T (\K + \I) ^{-1} \z } \nonumber \\ 
& \qquad\qquad\qquad \textstyle{ + \sum_{n=1}^{N} \log \Theta(y_n z_n) + c_2 ) } \ , \label{eq:gpc}
\end{align}
where $c_2 = \frac{N}{2} \log 2 \pi - \frac{1}{2} \log |\K + \I|$.
Uncertainty is shifted from the likelihood to the prior between these two representations.

In the move-step, we employ a parameter-free Gibbs sweep,
with its variances being either $1 / [\K^{-1}]_{ii}$ for (\ref{eq:gpc-x}), or $1 / [(\K+\I)^{-1}]_{ii}$ in the case of (\ref{eq:gpc}).
If we introduce the scaling of the covariance function in $\K= \sigma^2 \K_0$, it is easy to see that the variance of the Gibbs sampler scales with $\sigma^2$ for both formulations when $\sigma^2 \gg 1$, but for $\sigma^2 \ll 1$ the variance scales with $\sigma^2$ for (\ref{eq:gpc-x}) and is constant
for (\ref{eq:gpc}).
Gibbs sampling from (\ref{eq:gpc}) is thus more widely applicable as the step-size will in general be larger. Furthermore, the 
representation (\ref{eq:gpc}) has the additional advantage as it is amenable to fast \emph{slice sampling}
and avoids the computation of inverse Gaussian cumulative density functions $\Phi^{-1}$.
Details about the move- and augmentation-steps are given in the Supplementary Material.

\subsection{Experimental results}

\begin{figure*}[t!]
%\vspace{-0.1cm}
\begin{center}
\includegraphics[width=0.9\textwidth]{figures/GPC-all.pdf}
\caption{
An extensive time-based comparison for GPC on the USPS 3-vs.-5 data set, using a highly correlated prior. From left to right, the evaluations are for
(a) ARM with $R = 10^2, i_{\max} = 100$;
(b) RM with $R = 10^2$;
(c*) AIS$q$-RMHMC using $B=12$;
(d) ARM with $R = 10^3, i_{\max} = 50$;
(e) RM with $R = 10^3$;
(f*) AIS$q$-RMHMC using $B = 120$;
(g*) AIS$q$-RMHMC using $B = 240$;
(h) ARM with $R = 10^3, i_{\max} = 50$;
(i) RM with $R = 10^3$;
(j) AIS-RMHMC using $B = 1200$;
(k*) AIS$q$-RMHMC using $B = 540$;
(l) AIS-RMHMC using $B = 2000$;
(m*) AIS$q$-HMC.
The dotted line indicates EP's approximation, and the solid line a second order correction to the EP solution.
A label that is starred indicates that an AIS method was aided by annealing from EP's $q(\x)$ to $p(\x | \y)$, and not from the prior, as is more commonly done.
}
\label{fig:gpc}
\end{center}
% \vskip -0.2in
\end{figure*} 

We evaluate the efficiency of ARM evaluated on the USPS 3-vs.-5 data set \cite{KussAssessing},
using a covariance function $K_{mn} = k(\bxi_m, \bxi_n) = \sigma^2 \exp(-\frac{1}{2} \| \bxi_m - \bxi_n\|^2 / \ell^2 )$ that correlates inputs $\bxi_m$ and $\bxi_n$ through a length scale $\ell = \exp(4.85)$ and amplitude parameter $\sigma = \exp(5.1)$.\footnote{ARM was evaluated on \citet{KussAssessing}'s entire $(\log \ell, \log \sigma)$-grid, of which this setting proved to be the hardest.}
%%
Our main basis for comparison is Annealed Importance Sampling (AIS) \cite{NealAIS} using
different versions of Hamiltonian Monte Carlo (HMC) methods for the transition kernel.
Such a highly correlated high-dimensional prior highlights some deficiencies in
a basic HMC method, where mixing can be slow due to a sample's leapfrog trajectory oscillating
up and down the sides of a valley of $\log p(\y | \x)^{\beta} p(\x)$, without actually progressing
through it.
In order to get a working HMC sampler for the problem, we derived a Riemann Manifold HMC
method (RMHMC) \cite{RMHMC} for GP models.
To our knowledge, this has not been done before, and as it would be of independent interest,
detailed pseudo-code is given in the Supplementary Material.
To further aid AIS with different HMC methods, we additionally let AIS anneal from
a Gaussian approximation $q(\x)$ to the GPC posterior, which was obtained by Expectation Propagation (EP), instead of the prior.

Fig.~\ref{fig:gpc} compares these methods' estimates of $\log Z$ to the computation time to obtain it. Broadly, we see that ARM makes better use of a computational budget than RM.
Secondly, as the only competitive versions of AIS with HMC have to rely on outside information through $q(\x)$, SMC methods, in the spirit of ``hot coupling''  \citep{Hamze05hotcoupling},
are unequivocally better workhorses for estimating normalizing constants in this context.
The details of the methods are:

{\bf ARM} in (a), (d) and (h) uses $i_{\max} = 50$ (100 for (a)), with $R_n^{(0)}=R = 10^2, 10^3, 10^4$ respectively. Residual resampling is done when $R_{\mathrm{eff}} < 0.9 R$.

{\bf RM} in (b), (e) and (i) uses two Gibbs sweeps in each move-step, with $R = 10^2, 10^3, 10^4$,
and does residual resampling only when $R_{\mathrm{eff}} < 0.9 R$.
The choice of two sweeps is made to approximately match the average number of sweeps in ARM, which is around 1.5.

{\bf AIS$q$+HMC} in (m*) runs AIS from the EP's $q(\x)$ at $\beta=0$ to $p(\x | \y)$
at $\beta = 1$ using intermediate distributions
\[ \textstyle{
p_{\beta}(\x) = \frac{1}{Z_{\beta}}[ \prod_n \Phi(y_n x_n) \cdot {\cal N}(\x ; \0, \K) ]^{\beta} q(\x)^{1 - \beta} \ .
} \]
Note that a starred label indicates that the estimates were aided by $q(\x)$.
A HMC transition kernel with $\tau_{\max} = 200$ leapfrog steps
is used at each $\beta \in [0,1]$ value.
AIS's $\beta$-grid is a geometric progression over $B = 400$ $\beta$-values.
Plot (m*) used a step size $\epsilon = 0.02$ per proposal; both $\tau_{\max}$ and $\epsilon$ were carefully tuned to the problem.
The simplest AIS-HMC version, which anneals from $p(\x)$ and not $q(\x)$, didn't obtain estimates inside the bounds of Fig.~\ref{fig:gpc}, and is excluded. 

{\bf AIS+RMHMC} in (j) and (l) anneals from $p(\x)$, and replaces HMC with a more advanced RMHMC
that uses $\epsilon = 0.1$ and $\tau_{\max} = 10$ per proposal at each $\beta$ value.

{\bf AIS$q$+RMHMC} in (c*), (f*), (g*) and (k*) anneals from $q(\x)$ using a RMHMC kernel
($\epsilon = 0.1, \tau_{\max} = 10$).

It is known that the EP estimate of $\log Z$ is remarkably accurate for this problem \cite{KussAssessing}, hence EP's $\log Z$ estimate and its a second-order corrected estimate
\cite{OpperPerturbative} are given for reference.

Our last observation is a practical one. ARM and RM are simple and tend to be more robust
than AIS with HMC or Metropolis-Hastings, as they have little dependence on external parameters.
HMC, on the other hand, relies on carefully tuned settings of $\epsilon$ and $\tau$,
or requires more complicated extensions like RMHMC used here, or approaches like the No-U-Turn sampler \cite{HoffmanNoUTurn}.




%\todo{
%Although approaches like the No-U-Turn sampler \cite{HoffmanNoUTurn}, in conjunction with Nesterov's dual averaging scheme
%\cite{Nesterov}, . It is empirically underscored by Figure \ref{fig:gps-vs-ais},
%and the discussion surrounding Figure \ref{fig:rbm_comp} for RBMs.
%}
%
%\todo{Results for R=1e2,1e3 and 1e4 are attached. Overall they are significantly better than what we had before, I think.}
%\todo{
%I have modified the number of sweeps used in our approach to 
%nsteps = sqrt( par.corr * nparticles / eff-samp ) + 1;
%where par.corr=50. This is because the theoretical formula assumes independent samples. The number of independent samples should roughtly be divided by the correlation length which I for now set to 50. Next up is an actual calculation of it based upon measuring the correlation length of the weights (or log weights) empirically. }


==> pt.tex <==
%!TEX root = main.tex

\section{Parallel Tempering} \label{sec:pt}

\todo{continue here}
\todo{By Marco: perhaps this section is beyond the scope of this note? Also, we have it already the appendix of the DSP paper..}

%%
\begin{equation} \label{eq:p}
p_{\beta}(\x) \defined \frac{1}{Z(\beta)} \Big( p(\y | \x) \cdot \prior(\x) \Big)^{\beta} q(\x)^{1 - \beta} \ .
\end{equation}
%%
In this setup
$\beta = 1$ recovers $p(\x | \y)$, and $\beta = 0$ recovers $q(\x)$, or the prior if $q(\x) = p(\x)$.
The purpose behind Eq.~\ref{eq:p} is the identity
%%
\begin{equation} \label{eq:id}
\int_0^1 d \log Z(\beta) = \log Z(1) - \log Z(0) = \log Z \ ,
\end{equation}
%%
from which the normalising constant $\log Z$ can be determined.
This identity forms the backbone of AIS, PT, and other related methods. One would anneal from
$q(\x)$ at $\beta = 0$, and gradually incorporate the posterior by increasing $\beta$ towards $\beta = 1$.
Consider Eq.~\ref{eq:id} in greater detail.
%%
\begin{align*}
\int_0^1 d \log Z(\beta)
& = \int_0^1 \frac{d \log Z(\beta)}{d \beta} d \beta \\
& = \int_0^1 \int p_{\beta}(\x) \log \frac{ p(\y | \x) p(\x)}{q(\x)} \, d \x \, d \beta \\
& = \int_0^1 \Ebb_{\beta} \left[ \log \frac{p(\y | \x) p(\x)}{q(\x)} \right] d \beta \\
\end{align*}

(explain the moment annealing idea too. not geometric schedule. chris maddison.)


